Lower Bounds for Finding Stationary Points II: First-Order Methods

We establish lower bounds on the complexity of finding $\epsilon$-stationary points of smooth, non-convex high-dimensional functions using first-order methods. We prove that deterministic first-order methods, even applied to arbitrarily smooth functions, cannot achieve convergence rates in $\epsilon$ better than $\epsilon^{-8/5}$, which is within $\epsilon^{-1/15}\log\frac{1}{\epsilon}$ of the best known rate for such methods. Moreover, for functions with Lipschitz first and second derivatives, we prove no deterministic first-order method can achieve convergence rates better than $\epsilon^{-12/7}$, while $\epsilon^{-2}$ is a lower bound for functions with only Lipschitz gradient. For convex functions with Lipschitz gradient, accelerated gradient descent achieves the rate $\epsilon^{-1}\log\frac{1}{\epsilon}$, showing that finding stationary points is easier given convexity.

==> sections/firstorder/numerology.tex <==
% Congrats, you've found the easter egg!

\paragraph{Rate numerology}

\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
Let $R_p = \Delta \Smp \epsilon^{-(p+1)/p}$ be the optimal rate for $p$th order methods and $p$th order smoothness. It turns out the we may express both our upper and lower bounds for first-order methods with 1,...,$p$-order smoothness as $R_1^{\alpha}R_p^{1-\alpha}$ for some $\alpha\in(0,1)$; it is obvious we can find such $\alpha$ to get the $\epsilon$ power right, but maybe less obvious that we also get the powers on the Lipschitz constants right at the same time. Moreover, it turns out that this $\alpha$ has interesting values both for both the CUPG achievable (and maybe optimal?) rates, and our (maybe optimal?) lower bounds. Let's call the CUPG rates $\bar{F}_p$, for $p=2,3$. Then, we have
\begin{equation*}
\alpha_{\rm CUPG} = \half
\mbox{, i.e.\ }
\bar{F}_p = R_1^{1/2}R_p^{1/2}
\end{equation*}
for $p=2,3$. That is, the CUPG rate is exactly geometric average of $R_1$ and $R_p$ and consequently the CUPG exponent is the arithmetic means of $2$ and $(p+1)/p$.  Letting $\ubar{F}_p$ be our lower bounds, we have
\begin{equation*}
\alpha_{{\rm LB},p} = \frac{p+1}{3p+1}
\mbox{, i.e.\ }
\ubar{F}_2 = R_1^{3/7}R_p^{4/7}
~\mbox{and}~
\ubar{F}_3 = R_1^{2/5}R_p^{3/5}.
\end{equation*}
While these exponents (rather like the lower bound exponent themselves) might appear pretty bizarre, they actually have a curious property
\begin{equation*}
\alpha_{{\rm LB},p}\text{ is the solution to }
2\cdot \alpha = \frac{p+1}{p} \cdot (1-\alpha).
\end{equation*}
That is, it is the  $\alpha$  that makes $R_1^\alpha$ and $R_p^{1-\alpha}$ contribute the same $\epsilon$ dependence! Moreover, for $p>3$ if we go back to the proof of Theorem~\ref{thm:final} and instead of doing our $r$ scaling trick we keep $r=1$ and let $\mu \propto \sigma^{p-1}$, the above expression for $\alpha_{{\rm LB},p}$ remains true for all $p$! 
I guess it might be a freak accident of numerology, but to me it suggest that there might be something more profound to the funky $\epsilon$ powers in our lower bounds. 

I so far couldn't put my finger on what exactly in our construction or scaling argument forces the $\epsilon$ contributions to be identical, but I think it might be worth figuring out. Anyway, this curious ``equal $\epsilon$ contribution'' phenomenon is the only reason I have for thinking that maybe our lower bound construction is tight.  

